Bayesian Methods for Trust in Collaborative Multi-Agent Autonomy

Multi-agent, collaborative sensor fusion is a vital component of a multi-national intelligence toolkit. In safety-critical and/or contested environments, adversaries may infiltrate and compromise a number of agents. We analyze state of the art multi-target tracking algorithms under this compromised agent threat model. We prove that the track existence probability test ("track score") is significantly vulnerable to even small numbers of adversaries. To add security awareness, we design a trust estimation framework using hierarchical Bayesian updating. Our framework builds beliefs of trust on tracks and agents by mapping sensor measurements to trust pseudomeasurements (PSMs) and incorporating prior trust beliefs in a Bayesian context. In case studies, our trust estimation algorithm accurately estimates the trustworthiness of tracks/agents, subject to observability limitations.

==> algorithms/agent-trust.tex <==
\begin{algorithm}
\caption{Agent trust estimation}\label{alg:agent-trust}
\begin{algorithmic}
\Require $\hat{X}_{k,t}$ tracks from agent $k$ at time $t$, $X_t=\{x_{j,t}\}$ tracks from centralized fusion, $\{p(\tau_j^c | \Rho_{j,1:t-1})\}$ trust distributions over tracks $j$
\Ensure $p(\tau_k^a | \Rho_{1:t-1}\}$, estimate of agent trust
\State $\Bar{p} \gets \varnothing$
\State \Comment{detection}
\State \Comment{miss}
\State $p \gets \inf \Bar{p}$
\end{algorithmic}
\end{algorithm}

==> algorithms/two-step-update.tex <==
\begin{algorithm}
\caption{Alternating two-step update}\label{alg:two-step-update}
\begin{algorithmic}
TODO
\end{algorithmic}
\end{algorithm}

==> figures/trust-outcomes-all.tex <==
\begin{figure}[th]
    \centering
    \includegraphics[width=0.8\linewidth]{charts/experiment_metrics.pdf}
    \caption{TT: True Track, FT: False Track; $N=100$ Monte Carlo trials with random objects/FPs. True tracks determined trusted with 2 or 3 observers, unknown trust with 1 observer. False tracks determined distrusted only with 3 observers.}
    \label{fig:trust-outcomes-all}
\end{figure}

==> tables/trust-results.tex <==
\newcounter{advs}
\setcounter{advs}{0}
\newcommand{\resulttable}[4]{
    \begin{minipage}{.5\linewidth}
    \centering
    \begin{tabular}{c|c}
        TODO & TODO \\
        \midrule
        #1 & #2 \\
        #3 & #4 \\
        \bottomrule
    \end{tabular}
    \subcaption*{Panel A: n=\theadvs\ advs.}
    \stepcounter{advs}
    \end{minipage}
}

\begin{table}[!t]
    \centering
    \caption{Results}
    \label{tab:results}
    \begin{tabular}{c c}
         \resulttable{1}{1}{1}{1} & \resulttable{1}{1}{1}{1} \\
         \resulttable{1}{1}{1}{1} & \resulttable{1}{1}{1}{1}
    \end{tabular}
\end{table}



% % ============
% \begin{table}[!t]
%     \centering
%     \caption{AV Configurations}
%     % \vspace{-10pt}
%     \label{tab:table_case_configs}
%     % ----------------------------------------------
%     % FIRST SUBTABLE: AV DETAILS
%     % ----------------------------------------------
%     \resizebox{\columnwidth}{!}{%
% \begin{tabular}{llllll}
% \toprule
%                  Num. &                                                       AV Case Name &     LiDAR &   Camera &                              Tracking & Fusion \\ \midrule
% \midrule
%        \ref{av:lidar} &                                                         Lidar-Only & PtPillars &      N/A &                               AB3DMOT &    N/A \\ \midrule
% \ref{av:cam-lidar-v1} &                \tworowsubtableleft{Cam-LiDAR Fusion at}{Detection} & PtPillars & FstrRCNN &                              EagerMOT &    N/A \\ \midrule
% \ref{av:cam-lidar-v2} & \tworowsubtableleft{Cam-LiDAR Fusion at}{Detection w/ Asym. Check} & PtPillars & FstrRCNN &                              EagerMOT &    N/A \\ \midrule
%          \ref{av:ttt} &                 \tworowsubtableleft{Cam-LiDAR Fusion at}{Tracking} & PtPillars &      PGD & \tworowsubtableleft{AB3DMOT}{ (each)} &    T2T \\ \midrule
% \bottomrule
% \end{tabular}
%     }
    % \subcaption*{Panel A: AV configurations.}
    % \vspace{-10pt}
    % ----------------------------------------------
    % SECOND SUBTABLE: ATTACKER DETAILS
    % ----------------------------------------------
%     \bigskip
%     \resizebox{\columnwidth}{!}{%
% \begin{tabular}{lll}
% \toprule
%                  Num. &                            Att. Case Name &                                                                                                                                        Subroutines \\ \midrule
% \midrule
%          \ref{att:fp} &                            False Positive &                             \tworowsubtableleft{\texttt{FindMissingAngles}, \texttt{GetPointMaskFromTrace}}{\texttt{InpaintMaskAsObjectFromTrace}} \\ \midrule
%   \ref{att:forreplay} &                            Forward Replay &                                                                                                                                                N/A \\ \midrule
%   \ref{att:revreplay} &                            Reverse Replay &                                                                                                                                                N/A \\ \midrule
%      \ref{att:remove} &                            Object Removal & \tworowsubtableleft{Object Detection, Tracking}{\tworowsubtableleft{\texttt{GetPointMaskFromObject}}{\texttt{InpaintMaskAsBackgroundFromContext}}} \\ \midrule
% \ref{att:frust-trans} & \tworowsubtableleft{Frustum}{Translation} &                                                                                                \tworowsubtableleft{Object Removal}{False Positive} \\ \midrule
% \bottomrule
% \end{tabular}

%     }
%     \subcaption*{Panel B: Attacker configurations.}
    % \vspace{-16pt}
% \end{table}
% ============

